Improving Long-Range Interactions in Graph Neural Simulators via Hamiltonian Dynamics

Learning to simulate complex physical systems from data has emerged as a promising way to overcome the limitations of traditional numerical solvers, which often require prohibitive computational costs for high-fidelity solutions. Recent Graph Neural Simulators (GNSs) accelerate simulations by learning dynamics on graph-structured data, yet often struggle to capture long-range interactions and suffer from error accumulation under autoregressive rollouts. To address these challenges, we propose Information-preserving Graph Neural Simulators (IGNS), a graph-based neural simulator built on the principles of Hamiltonian dynamics. This structure guarantees preservation of information across the graph, while extending to port-Hamiltonian systems allows the model to capture a broader class of dynamics, including non-conservative effects. IGNS further incorporates a warmup phase to initialize global context, geometric encoding to handle irregular meshes, and a multi-step training objective that facilitates PDE matching, where the trajectory produced by integrating the port-Hamiltonian core aligns with the ground-truth trajectory, thereby reducing rollout error. To evaluate these properties systematically, we introduce new benchmarks that target long-range dependencies and challenging external forcing scenarios. Across all tasks, IGNS consistently outperforms state-of-the-art GNSs, achieving higher accuracy and stability under challenging and complex dynamical systems. Our project page: https://thobotics.github.io/neural_pde_matching.

==> tikz_colors.tex <==
\definecolor{tabblue}{RGB}{31, 119, 180}
\definecolor{taborange}{RGB}{255, 127, 14}
\definecolor{tabgreen}{RGB}{44, 160, 44}
\definecolor{tabred}{RGB}{214, 39, 40}
\definecolor{tabpurple}{RGB}{148, 103, 189}
\definecolor{tabbrown}{RGB}{140, 86, 75}
\definecolor{tabpink}{RGB}{227, 119, 194}
\definecolor{tabgray}{RGB}{127, 127, 127}
\definecolor{tabolive}{RGB}{188, 189, 34}
\definecolor{tabcyan}{RGB}{23, 190, 207}
\definecolor{lightblue}{RGB}{173, 216, 230}
\definecolor{sandybrown}{RGB}{244, 164, 96}
\definecolor{darkgrey}{RGB}{169, 169, 169}
\definecolor{dimgrey}{RGB}{105, 105, 105}
\definecolor{olivedrab}{RGB}{107, 142, 35}
\definecolor{darkviolet}{RGB}{148, 0, 211}
\definecolor{darkgoldenrod}{RGB}{184, 134, 11}
\definecolor{darkblue}{RGB}{0, 0, 139}
\definecolor{orchid}{RGB}{218, 112, 214}

\definecolor{blue}{RGB}{31, 119, 180}  % tv_hdgn_no_damping_no_forcing
\definecolor{orange}{RGB}{255, 127, 14}  % tv_hdgn_no_damping
\definecolor{green}{RGB}{44, 160, 44}  % tv_hdgn_no_forcing
\definecolor{red}{RGB}{214, 39, 40}  % tv_hdgn
\definecolor{purple}{RGB}{214, 39, 40}  % tv_hdgn_no_geom_enc
